Identification over Permutation Channels

We study message identification over a q-ary uniform permutation channel, where the transmitted vector is permuted by a permutation chosen uniformly at random. For discrete memoryless channels(DMCs), the number of identifiable messages grows doubly exponentially. Identification capacity, the maximum second-order exponent, is known to be the same as the Shannon capacity of the DMC. Permutation channels support reliable communication of only polynomially many messages. A simple achievability result shows that message sizes growing as 2^{\epsilon_nn^{q-1}} are identifiable for any \epsilon_n\rightarrow0. We prove two converse results. A ``soft'' converse shows that for any R>0, there is no sequence of identification codes with message size growing as 2^{Rn^{q-1}} with a power-law decay (n^{-\mu}) of the error probability. We also prove a ``strong" converse showing that for any sequence of identification codes with message size 2^{R_n n^{q-1}}, where R_n\rightarrow\infty, the sum of type I and type II error probabilities approaches at least 1 as n\rightarrow\infty. To prove the soft converse, we use a sequence of steps to construct a new identification code with a simpler structure which relates to a set system, and then use a lower bound on the normalized maximum pairwise intersection of a set system. To prove the strong converse, we use results on approximation of distributions. The achievability and converse results are generalized to the case of coding over multiple blocks. We finally study message identification over a q-ary uniform permutation channel in the presence of causal block-wise feedback from the receiver, where the encoder receives an entire n-length received block after the transmission of the block is complete. We show that in the presence of feedback, the maximum number of identifiable messages grows doubly exponentially, and we present a two-phase achievability scheme.

==> approximation_RV.tex <==

Towards proving Theorem \ref{thm:converse}B, we use a result on approximation of probability distributions with distributions having certain ``resolution''~\cite{koga2002information,han1993approximation}.

The variational distance between the two random variables $X,Y$ taking values from the set $\cZ$ and having distributions $P_X$ and $P_Y$ respectively,  is defined as
    \begin{align}
        d(X,Y) &\coloneqq \sum_{z \in \cZ} |P_X(z)-P_Y(z)|.
    \end{align}
Unless otherwise specified, we shall use $d(P_X,P_Y)$ and $d(X,Y)$ interchangeably.
For any random variable $Y$, the following lemma guarantees the existence of an approximating distribution of a certain resolution.
The lemma is a special case of \cite[Lemma $2.1.1$]{koga2002information}. The proof, which also specializes the proof of \cite[Lemma $2.1.1$]{koga2002information}, is given in Appendix~\ref{sec:pf_approximation_lemma} for completeness.

\begin{lemma}\label{lemma:approx output dist}
	For any positive integer $N$, and any random variable $Y$ taking values in $[N]$, and arbitrary constants $\alpha>a>0$,
	 there exists a mapping $\phi:[N^{\alpha}] \rightarrow [N]$ that satisfies  
	\begin{align}
		d(Y,&\phi(U_{N^{\alpha}})) \le 2 \times  \left\{N^{-(\alpha-a)}+ N^{-(a-1)} \right\}
	\end{align}
	where 
 $U_{N^{\alpha}}$ is the uniform random variable on $[N^{\alpha}]$. 
\end{lemma}











==> pf_theorem_stronger.tex <==
{\it Proof of Theorem~\ref{thm:converse}B:}

Consider a given sequence of $(n_i,2^{Rn_i^{q-1}\log n_i},\lambda_{1,i}, \lambda_{2,i})$ ID codes for  \bupcq  with  $n_i \rightarrow \infty$. Recall that $N_i$ is the number of type classes in $\cA_q^{n_i}$.
For each $i$,  using Lemma \ref{lemma: permutation to noiseless}, we construct an $(N_i, 2^{Rn_i^{q-1}\log n_i},\lambda_{1,i}, \lambda_{2,i})$ ID code for \noiselessNi with stochastic decoders.  We will now show that for such a sequence of codes, $\liminf_{i \rightarrow \infty} (\lambda_{1,i}+\lambda_{2,i}) \ge 1$. 


    Fix an $i$. The total variational distance between any two encoding distributions $Q_j^{i}, Q_k^{i}$ is related to the error probability  $\lambda_i$ as follows. For all $j \neq k$, we have
    \begin{align}
        d(Q_j^i,Q_k^i) & = \sum_{\bx \in [N_i]} |Q_j^i(x)-Q_k^i(x)| \notag \\
	&\ge  \sum_{\bx \in [N_i]} P_j^i(1|\bx) |Q_j^i(x)-Q_k^i(x)| \notag \\
        &\ge  \bigg(\sum_{\bx \in [N_i]} P_j^i(1|\bx)Q_j^i(x) 
        -  \sum_{\bx \in [N_i]} P_j^i(1|\bx)Q_k^i(x) \bigg)  \notag \\
	&=1-\lambda_{i,j\not\rightarrow j}-\lambda_{i,k\rightarrow j}\\
	&\ge  1-\lambda_{1,i} - \lambda_{2,i},
    \end{align}
    i.e.,
    \begin{align} \label{eq: lambda_n and TV distance}
        \lambda_{1,i}+\lambda_{2,i} \ge 1-d(Q_j^i,Q_k^i), \hspace{.2cm} \forall j \neq k, 
    \end{align}

    

Now we take a constant $R'$ satisfying $0< R'< \frac{R}{q-1}$ and fix  $1<a<\alpha<1+R'$. 
Consider a fixed $i$.
By Lemma \ref{lemma:approx output dist}, for every $j \in [2^{Rn_i^{q-1}\log n_i}]$, there exists a mapping $\phi_j^{(i)}:[N_i^{\alpha}] \rightarrow [N_i]$  such that the random variable $\tilde{Y}_i(j) \coloneqq \phi_j^{(i)}(U_{N_i^{\alpha}})$ satisfies 
\begin{align}
	d\left(Q_j^i,Q_{\tilde{Y}_i(j)}\right) \le \delta_i,
\end{align}
where $\delta_i \coloneqq 2 \times \left( N_i^{-(\alpha-a)}+N_i^{-(a-1)}\right)$. Since $\alpha>a>1$, $\delta_{i}\rightarrow 0$ as $i \rightarrow \infty$.

 The total number of distinct $N_i^{\alpha}$-type distributions on $[N_i]$ is upper bounded by
 \begin{align}
     \binom{N_i^{\alpha}+N_i-1}{N_i-1} 
     &\le \frac{N_i^{\alpha(N_i-1)}}{(N_i-1)!}\left(1+\frac{N_i-1}{N_i^{\alpha}}\right)^{N_i-1}\notag\\
     &\le \frac{N_i \cdot N_i^{\alpha(N_i-1)}}{N_i!}\cdot 2^{N_i}\notag \\
     &\stackrel{(a)}{\le}(2e)^{N_i}  \times 
     \frac{N_i^{[\alpha(N_i-1)+1]}}{N_i^{N_i}}\notag \\
     &=N_i^{\{ \alpha N_i -\alpha +1 -N_i+N_i\log_{N_i} (2e) \}}\notag \\
     &=N_i^{N_i\left(\alpha -1 +\frac{\log (2e)}{\log  N_i}-\frac{\alpha-1}{N_i} \right)}. \label{eq:bound1}
 \end{align}
Here $(a)$ follows from Stirling's approximation  $N_i! \ge \left(\frac{N_i}{e}\right)^{N_i}$.
For large enough $i$ (and hence $N_i$), \eqref{eq:bound1} can be further upper bounded by 
\begin{align*}
    N_i^{N_iR'} &=2^{R'N_i\log N_i}\\
    &\leq 2^{R_i''n_i^{q-1} \log n_i},
\end{align*}
 where
$$
R_i'' \coloneqq R'(q-1)\left(1+\frac{q-1}{n_i}\right)^{q-1}\left(1+\frac{\log \left( 1+\frac{q-1}{n_i}\right)}{\log n_i} \right).
$$ 
Here we have used the bound (see \eqref{eq:Nbounds})
$$
N_i \le (n_i+q-1)^{(q-1)}=n_i^{q-1}\left(1+ \frac{q-1}{n_i} \right)^{q-1}.
$$ 
Note that $R_i'' \rightarrow R'(q-1)< R$ as $i\rightarrow \infty$ (and hence $n_i \rightarrow \infty$). Hence $R_i'' < R$ for large enough $i$.
Hence, $\exists I$ such that for each $i>I$, there exist at least one pair $(j,k)$ with $j\neq k$ and $Q_{\tilde{Y}_i(j)}=Q_{\tilde{Y}_i(k)}$ and  we have
\begin{align}
	d(Q_j^i,Q_k^i)&\le d\left(Q_j^i,Q_{\tilde{Y}_i(j)}\right)+d\left(Q_k^i,Q_{\tilde{Y}_i(j)}\right)\\
	&= d\left(Q_j^i,Q_{\tilde{Y}_i(j)}\right)+ d\left(Q_k^i,Q_{\tilde{Y}_i(k)}\right)\\
	&\le 2 \delta_i. \label{eq:TV_lower_bound}
\end{align}
By combining \eqref{eq: lambda_n and TV distance} and \eqref{eq:TV_lower_bound} we have
\begin{align}
    \lambda_{1,i}+\lambda_{2,i} \ge 1-2\delta_{i}.
\end{align}
Since $\delta_{i}\rightarrow 0$ as $i \rightarrow \infty$, it follows that
\begin{align}
    \liminf_{i \rightarrow \infty} (\lambda_{1,i}+\lambda_{2,i}) \geq 1.
\end{align}
This completes the proof of Theorem \ref{thm:converse}B.


